Mid-IR Variability and Dust Reverberation Mapping of Low-$z$ Quasars. I. Data, Methods and Basic Results

The continued operation of the Wide-field Infrared Survey Explorer (WISE) combined with several ground-based optical transient surveys (e.g., CRTS, ASAS-SN and PTF) offer an unprecedented opportunity to explore the dust structures in luminous AGNs. We use these data for a mid-IR dust reverberation mapping (RM) study of 87 archetypal Palomar-Green quasars at $z\lesssim0.5$. To cope with various contaminations of the photometry data and the sparse time sampling of the light curves, procedures to combine these datasets and retrieve the dust RM signals have been developed. We find $\sim$70% of the sample (with a completeness correction, up to 95%) have convincing mid-IR time-lags in the WISE W1 ($\sim3.4~\mu m$) and W2 ($\sim4.5~\mu m$) bands and they are proportional to the square root of the AGN luminosity. Combined with previous K-band ($\sim2.2~\mu m$) RM results in the literature, the inferred dust emission size ratios are $R_{K}:R_{W1}:R_{W2}=0.6:1:1.2$. Under simple assumptions, we put preliminary constraints on the projected dust surface density at these bands and reveal the possibly different torus structures among hot-dust-deficient, warm-dust-deficient and normal quasars from the reverberation signals. With multi-epoch Spitzer data and later WISE photometry, we also explore AGN IR variability at 10--24 $\mu m$ over a 5-year time-scale. Except for blazars and flat-spectrum radio sources, the majority of AGNs have typical variation amplitudes at 24 $\mu m$ no more than 10% of that in the W1 band, indicating the dust reverberation signals damp out quickly at longer wavelengths. In particular, steep-spectrum radio quasars also lack strong 24 $\mu m$ variability, consistent with the unification picture of radio-loud AGN.

==> table2_full_online.tex <==
2MASX J00070361+1554240	& 0.114	& 3194.8	&	63.5	&	0.7	&		&	RQ	\\
	&  &	4676.2	&	62.9	&	0.7	&	0.6	&		\\
	&  &	5376$^a$	&	63.3	&	2.6	&	0.2	&		\\
PG0026+129	&  0.142 &	3747.4	&	43.2	&	0.7	&		&	RQ	\\
	&  &	4677.8	&	43.2	&	0.7	&	0.0	&		\\
	&  &	5382	&	44.1	&	3.8	&	0.2	&		\\
2MASS J00300421-2842259	& 0.278  &	3550.2	&	125.1	&	1.0	&		&	RQ, IRASF00275-2859	\\
	&  &	4675.4	&	124.7	&	1.0	&	0.3	&		\\
	&  &	5362	&	122.7	&	3.9	&	0.5	&		\\
2MASS J00411870+2816408	& 0.194 &	3195.3	&	74.5	&	0.8	&		&	RQ	\\
	&  &	4514.7	&	73.6	&	0.8	&	0.9	&		\\
	&  &	5392	&	76.6	&	2.5	&	1.2	&		\\
2MASX J00505570+2933281	& 0.136  &	3218.3	&	58.0	&	0.6	&		&		\\
	&  &	4514.7	&	57.3	&	0.7	&	0.8	&		\\
	&  &	5394	&	57.3	&	2.3	&	0.0	&		\\
PG0052+251	& 0.154  &	3217.8	&	68.7	&	0.7	&		&	RQ, W4 high due to strong 18 $\mu$m feature$^b$	\\
	&  &	4509.2	&	68.9	&	0.7	&	0.2	&		\\
	&  &	5393	&	76.0	&	2.4	&	2.9	&		\\
SDSSJ005621.72+003235.6	& 0.484 &	3582.8	&	17.6	&	0.6	&		&	RI	\\
	&  &	4330.4	&	17.5	&	0.6	&	0.1	&		\\
	&  &	5384	&	19.1	&	1.5	&	1.1	&		\\
3C29	&0.045  &	3223.5	&	6.0	&	0.5	&		&	RL, SSRQ$^c$	\\
	&  &	4336	&	5.5	&	0.6	&	0.6	&		\\
	&  &	4869.1	&	6.3	&	0.6	&	1.0	&		\\
	&  &	5384	&	6.9	&	1.4	&	0.7	&		\\
3C31	& 0.017  &	3365.5	&	21.4	&	0.5	&		&	RL, SSRQ	\\
	&  &	4512.7	&	21.6	&	0.5	&	0.3	&		\\
	&  &	4869.7	&	21.0	&	0.5	&	0.8	&		\\
	&  &	5398	&	20.0	&	1.2	&	1.1	&		\\
2MASS J01083514+2148184  & 0.285	&	3217.8	&	74.9	&	0.8	&		&	RQ	\\
	&  &	4509.2	&	74.7	&	0.8	&	0.2	&		\\
	&  &	5395	&	77.4	&	2.8	&	0.9	&		\\
3C33.1	&  0.181 &	3294.7	&	44.3	&	0.5	&		 &	RL, SSRQ	\\
	&  &	4397.4	&	42.6	&	0.5	&	2.5	&		\\
	&  &	4796.4	&	42.8	&	0.5	&	2.2	&		\\
	&  &	5240	&	44.2	&	1.6	&	0.6	&		\\
SDSSJ012341.47+004435.9	& 0.399 &	3747.2	&	8.6	&	0.6	&		&	RI	\\
	&  &	4335.9	&	8.5	&	0.6	&	0.1	&		\\
	&  &	5390	&	8.4	&	0.9	&	0.1	&		\\
2MASX J01291051-2141572	& 0.094  &	3747.9	&	167.3	&	1.3	&		&	RQ, IRASF01267-2157	\\
	&  &	4676.2	&	167.3	&	1.3	&	0.1	&		\\
	&  &	5384	&	162.7	&	5.2	&	0.9	&		\\
3C47	& 0.425 &	3399.5	&	33.2	&	0.7	&		&	RL, SSRQ	\\
	&  &	4512.6	&	33.2	&	0.6	&	0.1	&		\\
	&  &	4869.7	&	33.2	&	0.6	&	0.1	&		\\
	&  &	5400	&	32.9	&	1.5	&	0.2	&		\\
3C48	& 0.367 &	3218.8	&	132.4	&	1.1	&		&	RL, SSRQ	\\
	&  &	4512.7	&	131.6	&	1.1	&	0.5	&		\\
	&  &	4869.7	&	132.0	&	1.1	&	0.3	&		\\
	&  &	5405	&	130.3	&	4.4	&	0.4	&		\\
PHL1092	& 0.396 &	3238.9	&	26.9	&	0.6	&		&	RQ \\
	&  &	4335.9	&	26.2	&	0.7	&	0.8	&		\\
	&  &	5395	&	27.2	&	1.3	&	0.7	&		\\
SDSSJ015716.92-005304.8	& 0.422  &	3365.8	&	4.6	&	0.5	&		&   RQ		\\
	&  &	4335.9	&	4.4	&	0.6	&	0.3	&		\\
	&  &	5396	&	2.9	&	0.9	&	1.5	&		\\
2MASS J01572104+1712481&  0.213  &	3618.4	&	31.1	&	0.6	&		&	RQ	\\
	&  &	4336.1	&	30.7	&	0.7	&	0.5	&		\\
	&  &	5403	&	30.3	&	1.5	&	0.3	&		\\
4C +15.05	&  0.405 & 	3784.6	&	6.3	&	0.7	&		&	RL, PKS0202+149, variable, FSRQ, blazar$^d$ 	\\
	&  &	4336.1	&	10.2	&	0.6	&	4.1	&		\\
	&  &	4873.6	&	9.8	&	0.6	&	3.8	&		\\
	&  &	5404	&	17.3	&	1.1	&	7.7	&		\\
2MASS J02153839-1510125	& 0.211  &	3748	&	140.5	&	1.1	&		&	IRAS F02132-1524	\\
	&  &	4335.8	&	138.6	&	1.1	&	1.2	&		\\
	&  &	5396	&	141.0	&	4.0	&	0.6	&		\\
2MASX J02215058+1327409	& 0.140  &	3244.2	&	110.8	&	1.0	&		&	RQ, IRAS F02191+1313	\\
	&  &	4336.1	&	109.9	&	1.1	&	0.6	&		\\
	&  &	5408	&	108.8	&	3.4	&	0.3	&		\\
3C61.1	& 0.188  &	3085.1	&	6.6	&	0.4	&		&	RL, SSRQ	\\
	&  &	4397.3	&	7.4	&	0.3	&	1.6	&		\\
	&  &	4796.5	&	7.4	&	0.3	&	1.6	&		\\
	&  &	5266	&		&		&		&		\\
2MASX J02343065+2438353 	& 0.310 &	3244.3	&	71.2	&	0.8	&		&		\\
	&  &	4512.5	&	70.7	&	0.8	&	0.5	&		\\
	&  &	5226	&		&		&		&	confused	\\
3C78	&  0.029 &	3399.8	&	24.8	&	0.6	&		&	RL, variable, SSRQ, blazar	\\
	&  &	4512.6	&	19.4	&	0.6	&	6.7	&		\\
	&  &	4881.1	&	18.8	&	0.5	&	7.7	&		\\
	&  &	5229	&	18.2	&	1.4	&	2.0	&		\\
3C84	& 0.018 &	3426.9	&	2846.9	&	20.0	&		&	RL, probably variable, FSRQ$^e$, NGC 1275	\\
	&  &	4537.8	&	2882.8	&	20.2	&	1.3	&		\\
	&  &	4913.6	&	2869.7	&	21.1	&	0.8	&		\\
	&  &	5240	&	2680.7	&	65.3	&	2.8	&		\\
2MASX J03474022+0105143	& 0.030  &	3264.3	&	465.8	&	3.3	&		&	RQ, IRASF03450+0055	\\
	&  &	4512.6	&	469.0	&	3.4	&	0.7	&		\\
	&  &	5237	&	468.6	&	13.1	&	0.0	&		\\
2MASS J03485765+1255474  &  0.210 &	3270.2	&	151.0	&	1.2	&		&	RI	\\
	&  &	4543.7	&	149.5	&	1.2	&	0.9	&		\\
	&  &	5240	&	144.1	&	5.1	&	1.1	&		\\
2MASS J04260071-5712017	&  &	3613	&	109.4	&	0.9	&		&	RQ, IRASF04250-5718	\\
	&  &	4362.7	&	109.7	&	0.9	&	0.2	&		\\
	&  &	5394	&	117.3	&	3.3	&	2.3	&		\\
Pictor A	& 0.035 &	3084.8	&	130.5	&	1.0	&		&	RL, variable, SSRQ, high freq flat spectrum core	\\
	&  &	4400.9	&	118.2	&	0.9	&	9.0	&		\\
	&  &	4796.5	&	121.0	&	0.9	&	6.9	&		\\
	&  &	5255	&	124.2	&	3.8	&	0.3	&		\\
PKS0558-504	& 0.137 &	3106.7	&	87.5	&	0.7	&		&	RL, FSRQ	\\
	&  &	4400.9	&	87.6	&	0.8	&	0.1	&		\\
	&  &	4832.5	&	86.8	&	0.7	&	0.8	&		\\
	&  &	5273	&	88.4	&	2.8	&	0.4	&		\\
3C171	& 0.238 &	3084.8	&	7.9	&	0.5	&		&	RL, SSRQ	\\
	&  &	4397.3	&	7.8	&	0.5	&	0.2	&		\\
	&  &	4796.5	&	7.7	&	0.4	&	0.3	&		\\
	&  &	5283	&	8.7	&	1.0	&	0.9	&		\\
2MASS J07580005+3920289	& 0.095 &	3828.7	&	217.2	&	1.6	&		&	RQ, IRASF07546+3928	\\
	&  &	4433.4	&	215.5	&	1.6	&	0.7	&		\\
	&  &	5296	&	224.4	&	6.7	&	1.3	&		\\
PG0804+761	& 0.100 &	3059.8	&	188.2	&	1.4	&		&	RQ	\\
	&  &	4397.3	&	189.7	&	1.4	&	0.8	&		\\
	&  &	5285	&	197.0	&	5.5	&	1.3	&		\\
PG0844+349	& 0.064 &	3105.4	&	92.3	&	0.9	&		&       RQ		\\
	&  &	4432.6	&	90.4	&	0.9	&	1.6	&		\\
	&  &	5306	&	95.9	&	3.2	&	1.7	&		\\
2MASS J09134545+4056282	& 0.441 &	3104.1	&	292.5	&	2.1	&		& RQ, IRASF09105+4108		\\
	&  &	4246.1	&	288.3	&	2.1	&	1.4	&		\\
	&  &	5311	&	283.6	&	7.9	&	0.6	&		\\
2MASX J09161046-6219296	& 0.057  &	3104.5	&	1012.3	&	7.1	&		&   RQ,	IRAS09149-6206	\\
	&  &	4512.2	&	1007.0	&	7.1	&	0.5	&		\\
	&  &	5376	&	981.8	&	26.8	&	0.9	&		\\
Hydra A	& 0.055 &	3129.8	&	9.2	&	0.4	&		&	RL, SSRQ	\\
	&  &	4604.5	&	9.0	&	0.4	&	0.3	&		\\
	&  &	4833.1	&	9.1	&	0.5	&	0.2	&		\\
	&  &	5328	&	8.9	&	1.0	&	0.2	&		\\
2MASSiJ0918486+211717	& 0.149 &	3105	&	93.3	&	0.9	&		&	RQ, variable, IRAS F09159+2129	\\
	&  &	4434.4	&	88.8	&	0.9	&	3.5	&		\\
	&  &	5321	&	90.3	&	3.3	&	0.4	&		\\
SDSS J092014.12+453157.3	& 0.402 &	3319	&	21.6	&	0.5	&		&		\\
	&  &	4251.1	&	20.8	&	0.6	&	1.1	&		\\
	&  &	5311	&	20.5	&	1.3	&	0.3	&		\\
3C219	& 0.175 &	3104.1	&	13.2	&	0.5	&		&	RL, SSRQ	\\
	&  &	4251.1	&	12.1	&	0.5	&	1.6	&		\\
	&  &	4831.5	&	12.7	&	0.4	&	0.9	&		\\
	&  &	5311	&	13.5	&	1.2	&	0.7	&		\\
SDSS J094636.42+205610.9 & 0.279  &	3502.4	&	41.7	&	0.7	&		&   RQ		\\
	&  &	4602.5	&	41.1	&	0.6	&	0.7	&		\\
	&  &	5325	&	43.0	&	2.1	&	0.9	&		\\
2MASS J09550454+1705564	& 0.138  &	3128.8	&	18.6	&	0.6	&		&		\\
	&  &	4606.7	&	18.6	&	0.6	&	0.0	&		\\
	&  &	5328	&	19.0	&	1.3	&	0.3	&		\\
PG0953+414	& 0.234  &	3319	&	42.3	&	0.6	&		&	RQ	\\
	&  &	4246.1	&	42.7	&	0.6	&	0.5	&		\\
	&  &	5319	&	44.9	&	2.0	&	1.1	&		\\
3C236	& 0.101  &	3107.3	&	18.3	&	0.5	&		&	RL, SSRQ	\\
	&  &	4246.1	&	17.5	&	0.5	&	1.1	&		\\
	&  &	4832.6	&	16.8	&	0.5	&	2.1	&		\\
	&  &	5324	&	16.8	&	1.3	&	0.6	&		\\
SDSS J102724.98+121919.7	& 0.231 &	3505.6	&	80.8	&	0.8	&		&	RQ	\\
	&  &	4639.4	&	80.5	&	0.9	&	0.3	&		\\
	&  &	5337	&	82.5	&	2.8	&	0.7	&		\\
SDSS J103951.48+643004.2	& 0.402  &	3313	&	37.3	&	0.5	&		&	RQ	\\
	&  &	4432.6	&	36.7	&	0.5	&	0.9	&		\\
	&  &	5312	&	36.0	&	1.5	&	0.5	&		\\
PG1048+342	& 0.167  &	3503.8	&	25.8	&	0.6	&		&   RQ		\\
	&  &	4246.1	&	25.1	&	0.5	&	0.9	&		\\
	&  &	5334	&	25.2	&	1.2	&	0.1	&		\\
2MASX J10514428+3539304	& 0.159 &	3128.8	&	31.7	&	0.6	&		&	RI	\\
	&  &	4251.1	&	31.9	&	0.6	&	0.3	&		\\
	&  &	5331	&	33.6	&	1.6	&	1.0	&		\\
3C249.1	& 0.312 &	3085.1	&	45.3	&	0.5	&		&	RL, SSRQ, PG 1100+772	\\
	&  &	4432.5	&	45.1	&	0.5	&	0.3	&		\\
	&  &	4796.7	&	44.9	&	0.5	&	0.6	&		\\
	&  &	5298	&	47.1	&	1.7	&	1.1	&		\\
SDSSJ110621.96+035747.1	& 0.242 &	3508.7	&	14.8	&	0.6	&		&		\\
	&  &	4256.1	&	14.8	&	0.6	&	0.0	&		\\
	&  &	5350	&	14.3	&	1.1	&	0.4	&		\\
SDSS J112048.06+421212.4	& 0.124  &	3503.7	&	2.7	&	0.5	&		&	RL, FSRQ	\\
	&  &	4251.1	&	3.0	&	0.5	&	0.5	&		\\
	&  &	4832.6	&	2.9	&	0.4	&	0.3	&		\\
	&  &	5334	&	2.5	&	1.0	&	0.3	&		\\
PG1119+120	& 0.050 &	3508.4	&	222.7	&	1.7	&		&	 RQ	\\
	&  &	4257	&	221.9	&	1.7	&	0.3	&		\\
	&  &	5350	&	224.1	&	6.6	&	0.3	&		\\
2MASX J11362642+7009268	& 0.045 &	3107.6	&	10.3	&	0.4	&		&	RL, variable, FSRQ, blazar, Mrk 180	\\
	&  &	4433.3	&	9.5	&	0.4	&	1.4	&		\\
	&  &	4797	&	9.7	&	0.4	&	1.0	&		\\
	&  &	5314	&	15.8	&	1.1	&	5.5	&		\\
3C264	& 0.022 &	3175	&	15.8	&	0.6	&		&	RL, SSRQ	\\
	&  &	4258.2	&	14.3	&	0.5	&	1.8	&		\\
	&  &	4880	&	14.7	&	0.5	&	1.4	&		\\
	&  &	5352	&	13.8	&	1.0	&	1.1	&		\\
SDSSJ115718.34+600345.6	& 0.490 &	3461	&	56.3	&	0.6	&		& RQ		\\
	&  &	4602.9	&	56.2	&	0.6	&	0.1	&		\\
	&  &	5327	&	54.9	&	1.9	&	0.7	&		\\
PG1202+281	& 0.165  & 	3508.3	&	79.8	&	0.8	&		& RQ		\\
	&  &	4511.2	&	78.0	&	0.7	&	1.7	&		\\
	&  &	5353	&	79.8	&	2.6	&	0.7	&		\\
PG1211+143	&  0.073 &	3546.9	&	242.9	&	1.8	&		&	RQ 	\\
	&  &	4513.5	&	241.2	&	1.8	&	0.7	&		\\
	&  &	4872.7	&	241.8	&	1.8	&	0.4	&		\\
	&  &	5361	&	248.0	&	7.6	&	0.8	&		\\
3C270	&0.007  &	3543	&	48.7	&	0.7	&		&	RL, probably variable, SSRQ	\\
	&  &	4513.5	&	48.3	&	0.7	&	0.4	&		\\
	&  &	4868.2	&	51.0	&	0.7	&	2.8	&		\\
	&  &	5366	&	44.9	&	2.1	&	2.1	&		\\
ON231	& 0.102  &	3509.9	&	54.5	&	0.6	&		&	RL, variable, FSRQ, blazar	\\
	&  &	4256.8	&	54.8	&	0.6	&	0.4	&		\\
	&  &	4882	&	63.5	&	0.7	&	9.9	&		\\
	&  &	5366	&	49.3	&	1.8	&	4.5	&		\\
3C272.1	& 0.003  & 	3157.4	&	38.4	&	0.6	&		&	RL, variable, FSRQ, M84	\\
	&  &	4293.4	&	38.2	&	0.6	&	0.2	&		\\
	&  &	4869.8	&	37.3	&	0.7	&	1.2	&		\\
	&  &	5364	&	31.9	&	1.4	&	4.1	&		\\
3C273	& 0.158  &	3175.4	&	503.6	&	3.6	&		&	RL, variable, FSRQ, blazar, PG 1226+023	\\
	&  &	4298	&	545.4	&	3.9	&	7.9	&		\\
	&  &	4869.8	&	646.3	&	4.6	&	24.4	&		\\
	&  &	5372	&	507.6	&	14.2	&	4.0	&		\\
3C274	& 0.004 &	3365.7	&	90.2	&	0.9	&		&	RL, variable, M87, high frequency radio core	\\
	&  &	4513.5	&	103.2	&	0.9	&	10.0	&		\\
	&  &	4869.8	&	82.8	&	0.8	&	16.4	&		\\
	&  &	5365	&	72.7	&	2.8	&	6.9	&		\\
PG1229+204	& 0.064  &	3547.7	&	146.7	&	1.2	&		&	RQ	\\
	&  &	4298.4	&	143.7	&	1.2	&	1.8	&		\\
	&  &	5364	&	145.8	&	4.5	&	0.5	&		\\
SDSS J123215.81+020610.0 & 0.481 &	3546	&	8.6	&	0.6	&		&		\\
	&  &	4294	&	8.1	&	0.6	&	0.6	&		\\
	&  &	5372	&	9.7	&	1.1	&	1.4	&		\\
SDSS J124210.61+331702.6	& 0.044 &	3508.3	&	195.3	&	1.5	&		& RQ, IRASF12397+3333	\\
	&  &	4256.9	&	193.2	&	1.5	&	1.0	&		\\
	&  &	5358	&	198.3	&	5.8	&	0.9	&		\\
3C277.1	& 0.320 &	3107.5	&	20.8	&	0.4	&		&	RL, SSRQ	\\
	&  &	4513	&	20.2	&	0.4	&	1.0	&		\\
	&  &	4832.3	&	19.9	&	0.4	&	1.5	&		\\
	&  &	5342	&	19.6	&	1.0	&	0.7	&		\\
3C277.3	& 0.086 &	3177.2	&	9.6	&	0.5	&		&	RL, SSRQ, Coma A	\\
	&  &	4513.5	&	9.7	&	0.5	&	0.2	&		\\
	&  &	4871.1	&	9.4	&	0.5	&	0.4	&		\\
	&  &	5365	&	10.1	&	0.9	&	0.6	&		\\
2MASS J12580745+2329216 & 0.258 &	3178.9	&	69.4	&	0.7	&		&	RQ	\\
	&  &	4513.1	&	69.1	&	0.7	&	0.3	&		\\
	&  &	5367	&	71.0	&	2.4	&	0.8	&		\\
2MASX J13000533+1632151	& 0.080  &	3194.3	&	156.5	&	1.3	&		&	RQ	\\
	&  &	4513.5	&	156.8	&	1.2	&	0.2	&		\\
	&  &	5382	&	165.5	&	5.8	&	1.5	&		\\
SDSSJ130128.77-005804.3	& 0.246 &	3540.1	&	10.6	&	0.6	&		&  RQ		\\
	&  &	4512.9	&	10.2	&	0.6	&	0.5	&		\\
	&  &	5349	&	12.0	&	1.0	&	1.7	&		\\
2MASX J13070062+2338052	& 0.275 &	3177.2	&	73.7	&	0.7	&		& RQ, IRAS 13045+2353		\\
	&  &	4513	&	73.4	&	0.7	&	0.3	&		\\
	&  &	5371	&	71.4	&	2.5	&	0.8	&		\\
PG1307+085	& 0.154 &	3197.6	&	67.6	&	0.8	&		& RQ	\\
	&  &	4294	&	66.9	&	0.7	&	0.7	&		\\
	&  &	5378	&	70.2	&	2.8	&	1.2	&		\\
3C284	& 0.240 &	3194.2	&	25.1	&	0.5	&		&	RL, SSRQ	\\
	&  &	4513.4	&	25.2	&	0.5	&	0.1	&		\\
	&  &	4874.5	&	24.6	&	0.5	&	0.8	&		\\
	&  &	5371	&	25.8	&	1.9	&	0.5	&		\\
PG1309+355	& 0.183  & 	3177.2	&	103.9	&	0.9	&		&	RL$^f$, FSRQ	\\
	&  &	4256.9	&	103.4	&	0.9	&	0.4	&		\\
	&  &	4871.7	&	103.8	&	0.9	&	0.3	&		\\
	&  &	5363	&	107.6	&	3.4	&	1.1	&		\\
SDSSJ132323.33-015941.9	& 0.350 &	3545.2	&	12.7	&	0.6	&		& RQ		\\
	&  &	4512.9	&	12.6	&	0.6	&	0.1	&		\\
	&  &	5384	&	12.4	&	1.1	&	0.2	&		\\
PG1322+659	& 0.168 &	3107.6	&	44.5	&	0.5	&		&  RQ		\\
	&  &	4512.4	&	43.5	&	0.5	&	1.4	&		\\
	&  &	5332	&	44.2	&	1.8	&	0.4	&		\\
NVSS J132439-073417	& -- &	3550.6	&	8.0	&	0.6	&		&  RQ		\\
	&  &	4294.4	&	8.0	&	0.6	&	0.0	&		\\
	&  &	5387	&	7.1	&	0.9	&	0.9	&		\\
3C293	& 0.045 &	3549.1	&	32.5	&	0.5	&		&	RL, SSRQ	\\
	&  &	4300.5	&	32.9	&	0.5	&	0.6	&		\\
	&  &	4871.7	&	33.1	&	0.6	&	0.8	&		\\
	&  &	5377	&	31.7	&	1.4	&	0.8	&		\\
PG1351+640	& 0.086  &	3707	&	417.7	&	3.0	&		&	RQ	\\
	&  &	4512.4	&	416.4	&	3.0	&	0.3	&		\\
	&  &	5341	&	420.3	&	11.8	&	0.3	&		\\
2MASS J13555019+2046144	& 0.196 &	3550.5	&	155.8	&	1.2	&		& RQ, IRASF13534+2100	\\
	&  &	4513	&	155.9	&	1.2	&	0.1	&		\\
	&  &	5382	&	157.2	&	4.5	&	0.3	&		\\
PG1354+213	& 0.300 &	3543.6	&	29.2	&	0.5	&		&   RQ		 \\
	&  &	4513	&	28.6	&	0.5	&	0.8	&		\\
	&  &	5384	&	30.3	&	1.4	&	1.2	&		\\
2MASS J14025120+2631175 & 0.187 &	3177.1	&	23.4	&	0.5	&		 &		\\
	&  &	4513	&	24.0	&	0.5	&	0.9	&		\\
	&  &	5383	&	25.6	&	1.2	&	1.3	&		\\
PG1402+261	& 0.164 &	3177.1	&	100.1	&	0.9	&		&  RQ		\\
	&  &	4513	&	101.3	&	0.9	&	1.0	&		\\
	&  &	5383	&	105.0	&	3.5	&	1.1	&		\\
PG1404+226	& 0.098 &	3549.3	&	27.0	&	0.5	&		&	RQ	\\
	&  &	4513	&	26.4	&	0.5	&	0.8	&		\\
	&  &	5385	&	29.3	&	1.5	&	2.0	&		\\
SDSSJ141315.30-014221.0	& 0.380  &	3782.7	&	15.8	&	0.6	&		& RQ		\\
	&  &	4512.8	&	15.5	&	0.7	&	0.3	&		\\
	&  &	5396	&	16.0	&	0.9	&	0.5	&		\\
PG1411+442	& 0.087 &	3508.1	&	119.1	&	1.0	&		&	RQ 	\\
	&  &	4512.4	&	118.0	&	0.9	&	0.8	&		\\
	&  &	5375	&	121.6	&	3.7	&	1.0	&		\\
3C296	& 0.025 &	3784.8	&	10.5	&	0.5	&		&	RL, SSRQ	\\
	&  &	4513.5	&	10.3	&	0.5	&	0.3	&		\\
	&  &	4881.6	&	10.3	&	0.6	&	0.3	&		\\
	&  &	5392	&	10.3	&	0.8	&	0.1	&		\\
PG1415+451	& 0.114 &	3508.1	&	57.8	&	0.6	&		&	RQ	\\
	&  &	4512.8	&	57.3	&	0.6	&	0.6	&		\\
	&  &	5374	&	59.1	&	2.1	&	0.8	&		\\
OQ530	& 0.153 &	3108	&	90.4	&	0.8	&		&	RL, variable, FSRQ, blazar	\\
	&  &	4512.8	&	91.1	&	0.8	&	0.6	&		\\
	&  &	4873.6	&	77.9	&	0.7	&	12.2	&		\\
	&  &	5361	&	74.5	&	2.4	&	4.9	&		\\
SDSS J142130.04+474728.6	& 0.073 &	3508.1	&	218.1	&	1.6	&		& RQ, IRASF14196+4801	\\
	&  &	4512.8	&	215.6	&	1.6	&	1.1	&		\\
	&  &	5370	&	219.3	&	6.4	&	0.6	&		\\
2MASS J14283260+4240209	& 0.129 &	3508.1	&	2.4	&	0.4	&		&	RL, FSRQ, H1426+428	\\
	&  &	4512.8	&	2.8	&	0.4	&	0.7	&		\\
	&  &	4873.6	&	2.4	&	0.4	&	0.7	&		\\
	&  &	5379	&	2.4	&	0.9	&	0.2	&		\\
PG1426+015	& 0.086  & 	3059.4	&	183.3	&	1.4	&		&	RQ	\\
	&  &	4329.9	&	182.5	&	1.4	&	0.4	&		\\
	&  &	5402	&	187.7	&	5.3	&	1.0	&		\\
PG1440+356	& 0.077 &	3790.4	&	175.7	&	1.3	&		&   RQ  	\\
	&  &	4513	&	175.2	&	1.3	&	0.3	&		\\
	&  &	5389	&	177.4	&	5.1	&	0.4	&		\\
3C303.1	& 0.267 &	3107.7	&	8.1	&	0.2	&		&	RL, variable, SSRQ	\\
	&  &	4401.2	&	7.2	&	0.2	&	3.0	&		\\
	&  &	4796.7	&	7.4	&	0.3	&	1.9	&		\\
	&  &	5310	&	7.6	&	0.7	&	0.0	&		\\
PG1444+407	& 0.267 &	3549.2	&	59.4	&	0.6	&		&   RQ	 	\\
	&  &	4512.8	&	59.2	&	0.6	&	0.2	&		\\
	&  &	5384	&	61.5	&	2.4	&	1.0	&		\\
3C305	& 0.042 &	3107.7	&	45.8	&	0.5	&		&	RL, SSRQ	\\
	&  &	4512.4	&	44.9	&	0.5	&	1.3	&		\\
	&  &	4832.7	&	45.2	&	0.5	&	0.8	&		\\
	&  &	5349	&	41.9	&	1.5	&	2.2	&		\\
2MASS J14533150+1353585	& 0.139 &	3058.1	&	118.8	&	1.0	&		&	RQ, IRAS 14511+1406	\\
	&  &	4539.5	&	117.6	&	1.0	&	0.9	&		\\
	&  &	5402	&	110.7	&	3.3	&	2.0	&		\\
2MASS J14560866+2750088	& 0.248 &	3549.2	&	26.8	&	0.5	&		&    RQ		\\
	&  &	4513	&	26.5	&	0.5	&	0.4	&		\\
	&  &	5396	&	26.6	&	1.2	&	0.1	&		\\
2MASS J15011320+2329082	& 0.258 &	3549.3	&	47.1	&	0.6	&		&	RQ	\\
	&  &	4513.3	&	47.7	&	0.6	&	0.7	&		\\
	&  &	5397	&	47.9	&	1.8	&	0.1	&		\\
2MASX J15011790+5455181 & 0.339 &	3400.1	&	8.5	&	0.4	&		&	RL, SSRQ	\\
	&  &	4250.6	&	8.5	&	0.4	&	0.0	&		\\
	&  &	5372	&	8.3	&	0.8	&	0.3	&		\\
PG1501+106	& 0.036 &	3060.8	&	417.1	&	3.0	&		&	RQ 	\\
	&  &	4330.4	&	410.3	&	2.9	&	1.6	&		\\
	&  &	5406	&	407.8	&	11.1	&	0.2	&		\\
PKS1510-08	& 0.360 &	3611.8	&	41.4	&	0.7	&		&	RL, variable, blazar, FSRQ\\
	&  &	4339.9	&	137.4	&	1.2	&	71.0	&		\\
	&  &	4913.5	&	141.1	&	1.2	&	71.1	&		\\
	&  &	5237	&	68.9	&	2.4	&	15.2	&		\\
3C315	& 0.108 &	3223.4	&	2.5	&	0.4	&		&	RL, SSRQ	\\
	&  &	4539.4	&	1.9	&	0.4	&	1.0	&		\\
	&  &	4913.5	&	2.2	&	0.4	&	0.5	&		\\
	&  &	5402	&		&		&	0.0	&		\\
PG1512+370	& 0.371 &	3084.6	&	31.1	&	0.5	&		&	RL, SSRQ 	\\
	&  &	4512.8	&	30.9	&	0.5	&	0.3	&		\\
	&  &	4880	&	30.7	&	0.5	&	0.6	&		\\
	&  &	5396	&	31.4	&	1.2	&	0.4	&		\\
2MASS J15165323+1900482	& 0.190 &	3194.3	&	127.3	&	1.0	&		&		\\
	&  &	4539.4	&	125.1	&	1.0	&	1.5	&		\\
	&  &	5405	&	128.9	&	4.1	&	0.9	&		\\
2MASS J15304948+2026049	& 0.216 &	3788.6	&	89.3	&	0.8	&		&  RQ, IRASF15285+2036	\\
	&  &	4539.4	&	89.4	&	0.8	&	0.1	&		\\
	&  &	5409	&	91.6	&	2.9	&	0.8	&		\\
PG1535+547	& 0.039 &	3081.7	&	73.8	&	0.7	&		&	RQ, variable	\\
	&  &	4512.4	&	70.5	&	0.7	&	3.6	&		\\
	&  &	5382	&	74.3	&	2.1	&	1.7	&		\\
2MASS J15430778+1937518	& 0.229 &	3084.6	&	81.5	&	0.7	&		& RQ		\\
	&  &	4539.4	&	80.3	&	0.8	&	1.1	&		\\
	&  &	5236	&	82.9	&	2.7	&	0.9	&		\\
3C323.1	& 0.264 &	3241.9	&	33.7	&	0.5	&		&	RL, SSRQ, PG 1545+210	\\
	&  &	4358.3	&	33.3	&	0.5	&	0.6	&		\\
	&  &	4913.4	&	33.4	&	0.6	&	0.4	&		\\
	&  &	5237	&	35.6	&	1.4	&	1.5	&		\\
3C327	& 0.104 &	3084.9	&	246.5	&	1.8	&		&	RL, SSRQ	\\
	&  &	4539.2	&	245.0	&	1.8	&	0.6	&		\\
	&  &	4913.5	&	243.0	&	1.8	&	1.4	&		\\
	&  &	5245	&	236.5	&	6.9	&	1.2	&		\\
PG1617+175	& 0.112 &	3466.9	&	48.3	&	0.6	&		&	RQ	\\
	&  &	4539.5	&	47.9	&	0.6	&	0.5	&		\\
	&  &	5247	&	50.4	&	1.9	&	1.3	&		\\
2MASS J16370022+2221140	& 0.211 &	3085.7	&	24.9	&	0.5	&		&	RQ	\\
	&  &	4372.4	&	25.3	&	0.5	&	0.6	&		\\
	&  &	5250	&	25.5	&	1.2	&	0.2	&		\\
2MASS J16373650+2543028	& 0.277 &	3085.7	&	37.9	&	0.5	&		&	RQ	\\
	&  &	4372.4	&	37.5	&	0.5	&	0.6	&		\\
	&  &	5250	&	37.9	&	1.8	&	0.2	&		\\
Mrk501	& 0.033 &	3106	&	69.9	&	0.7	&		&	RL, variable, blazar, FSRQ	\\
	&  &	4539.4	&	49.7	&	0.6	&	23.7	&		\\
	&  &	4913.5	&	49.7	&	0.6	&	22.7	&		\\
	&  &	5250	&	54.2	&	1.9	&	1.2	&		\\
3C349	& 0.205 &	3103.2	&	6.3	&	0.4	&		&	RL, SSRQ	\\
	&  &	4539.4	&	5.9	&	0.4	&	0.7	&		\\
	&  &	4913.5	&	6.1	&	0.4	&	0.4	&		\\
	&  &	5249	&		&		&		&		\\
2MASS J16593976+1834367	& 0.171 &	3085.3	&	134.3	&	1.1	&		&	RQ	\\
	&  &	4372.4	&	134.5	&	1.1	&	0.1	&		\\
	&  &	5258	&	136.7	&	3.8	&	0.6	&		\\
PG1700+518	& 0.289 &	3108	&	178.2	&	1.3	&		&	RQ	\\
	&  &	4541	&	176.2	&	1.3	&	1.1	&		\\
	&  &	5244	&	176.2	&	4.7	&	0.0	&		\\
3C351	& 0.372 &	3105.2	&	104.1	&	0.9	&		&	RL, SSRQ, PG 1704+608	\\
	&  &	4400	&	101.6	&	0.8	&	2.1	&		\\
	&  &	4796.7	&	101.5	&	0.8	&	2.2	&		\\
	&  &	5394	&	99.5	&	2.9	&	1.0	&		\\
2MASS J17144278+2602485	& 0.163 &	3060	&	25.9	&	0.5	&		&		\\
	&  &	4372.4	&	25.9	&	0.4	&	0.0	&		\\
	&  &	5260	&	26.2	&	1.3	&	0.2	&		\\
Mrk506	& 0.043 &	3611.7	&	82.6	&	0.7	&		&	RQ, variable, FS radio core	\\
	&  &	4372.4	&	78.6	&	0.7	&	4.0	&		\\
	&  &	5263	&	75.7	&	2.6	&	1.1	&		\\
4C34.47	& 0.206 &	3465.7	&	56.3	&	0.6	&		&	RL, FSRQ	\\
	&  &	4604.9	&	54.8	&	0.6	&	1.8	&		\\
	&  &	5263	&	58.1	&	1.9	&	1.7	&		\\
3C371	& 0.051  &	3105.2	&	147.6	&	1.1	&		&	RL, variable, blazar, FSRQ	\\
	&  &	4401.2	&	100.0	&	0.8	&	34.4	&		\\
	&  &	4796.7	&	119.2	&	0.9	&	19.4	&		\\
	&  &	5258	&	98.6	&	2.8	&	8.2	&		\\
3C381	&  0.161  &	3106	&	47.1	&	0.5	&		&	RL, SSRQ	\\
	&  &	4402.7	&	45.3	&	0.5	&	2.5	&		\\
	&  &	4796.7	&	45.1	&	0.5	&	2.7	&		\\
	&  &	5296	&	47.5	&	1.8	&	1.0	&		\\
3C388	& 0.091 &	3106.1	&	2.8	&	0.3	&		&	RL, SSRQ	\\
	&  &	4402.7	&	1.9	&	0.3	&	2.1	&		\\
	&  &	4796.7	&	2.1	&	0.3	&	1.6	&		\\
	&  &	5299	&	1.5	&	0.9	&	0.9	&		\\
3C401	& 0.201 &	3297.1	&	1.4	&	0.3	&		&	RL, SSRQ	\\
	&  &	4339.7	&	1.1	&	0.3	&	0.6	&		\\
	&  &	4796.7	&	1.2	&	0.3	&	0.5	&		\\
	&  &	5351	&	1.9	&	1.0	&	0.7	&		\\
Cygnus A	& 0.056 &	3295.6	&	674.1	&	4.8	&		&	RL, SSRQ	\\
	&  &	4329.3	&	667.3	&	4.7	&	1.0	&		\\
	&  &	4796.7	&	667.1	&	4.7	&	1.1	&		\\
	&  &	5327	&	633.1	&	14.8	&	2.4	&		\\
PKS2005-489	& 0.071 &	3103.7	&	78.0	&	0.7	&		&	RL, variable, FSRQ, blazar	\\
	&  &	4400.9	&	77.9	&	0.8	&	0.1	&		\\
	&  &	5301	&	56.4	&	2.2	&	9.6	&		\\
2MASS J20481724+1936560	& 0.181 &	3296.9	&	435.8	&	3.1	&		&	RQ, IRASF20460+1925	\\
	&  &	4433.3	&	433.9	&	3.1	&	0.4	&		\\
	&  &	5330	&	428.1	&	10.7	&	0.5	&		\\
PG2130+099	& 0.062 &	3314.1	&	301.6	&	2.2	&		&	RQ	\\
	&  &	4433.3	&	300.4	&	2.2	&	0.4	&		\\
	&  &	5338	&	304.4	&	8.1	&	0.5	&		\\
PKS2155-304	& 0.116 &	3297	&	110.9	&	1.0	&		&	RL, variable, FSRQ, blazar	\\
	&  &	4431.6	&	202.7	&	1.6	&	50.5	&		\\
	&  &	4796.8	&	140.4	&	1.2	&	32.3	&		\\
	&  &	5331	&	94.0	&	3.6	&	15.6	&		\\
4C31.63	& 0.295 &	3315.5	&	69.4	&	0.6	&		&	RL, variable, FSRQ, blazar\\
	&  &	4433.8	&	74.4	&	0.7	&	5.4	&		\\
	&  &	4831.1	&	75.1	&	0.7	&	6.2	&		\\
	&  &	5356	&	72.4	&	2.6	&	0.2	&		\\
PG2209+184	& 0.070 &	3316.8	&	20.5	&	0.5	&		&	RL, variable, FSRQ	\\
	&  &	4676.7	&	21.4	&	0.5	&	1.4	&		\\
	&  &	4825.8	&	27.1	&	0.4	&	10.5	&		\\
	&  &	5350	&	21.4	&	1.4	&	1.1	&		\\
2MASS J22220221+1952316	& 0.366 &	3178.1	&	37.6	&	0.5	&		&	RQ	\\
	&  &	4676.7	&	37.5	&	0.5	&	0.1	&		\\
	&  &	5356	&	39.2	&	1.6	&	1.0	&		\\
2MASXi J2222211+195947	& 0.209 &	3197.8	&	48.0	&	0.6	&		&		\\
	&  &	4676.7	&	47.9	&	0.6	&	0.1	&		\\
	&  &	5356	&	48.8	&	2.0	&	0.4	&		\\
2MASX J22255423+1958372	& 0.147 &	3178.1	&	43.1	&	0.6	&		&	RQ	\\
	&  &	4676.7	&	43.1	&	0.6	&	0.0	&		\\
	&  &	5356	&	43.6	&	1.9	&	0.3	&		\\
PKS2247+14	& 0.235 &	3548.2	&	23.2	&	0.6	&		&	RL, FSRQ	\\
	&  &	4675.4	&	22.7	&	0.5	&	0.7	&		\\
	&  &	4830.2	&	23.0	&	0.5	&	0.4	&		\\
	&  &	5362	&	24.6	&	1.4	&	1.2	&		\\
2MASX J23083397+0521293	& 0.173  &	3345.9	&	417.0	&	3.0	&		&	RQ, IRASF23060+0505	\\
	&  &	4676.7	&	415.0	&	3.0	&	0.5	&		\\
	&  &	5361	&	403.8	&	11.6	&	1.0	&		\\
2MASX J23444953+1221430	& 0.199 &	3215.1	&	55.9	&	0.6	&		&		\\
	&  &	4675.3	&	56.5	&	0.7	&	0.6	&		\\
	&  &	5371	&	58.4	&	2.1	&	0.9	&		\\
SDSSJ235818.86-000919.4	& 0.402  &	3344	&	6.3	&	0.6	&		&		\\
	&  &	4469.1	&	6.0	&	0.6	&	0.4	&		\\
	&  &	5369	&	5.4	&	1.2	&	0.5	&		


==> table5_full_online.tex <==
 PG 0003+158 &  53721.5 &   13.62 &   0.88  &	      &        &  53721.5 &  24.41 &   2.06 &        &        &                \\
             &  55376.1 &   13.96 &   0.34  &  -0.36  &  0.03  &  55376.1 &  25.02 &   1.24 &  -0.25 &   0.03 &\\
 PG 0003+199 &  53559.2 &  175.20 &   3.62  &         &        & $\cdots$ &$\cdots$&$\cdots$&        &        &\\
             &  55377.8 &  191.29 &   2.53  &  -3.65  &  0.10  &  55377.8 & 280.42 &   5.60 &        &        &\\
 PG 0007+106 &  53721.3 &   74.01 &   2.75  &         &        &  53721.3 & 153.34 &   3.90 &        &        &\\
             &  55375.0 &   64.94 &   1.00  &   3.10  &  0.15  &  55375.0 & 126.65 &   2.79 &   5.56 &   0.23 &  variable, FSRQ\\
 PG 0026+129 &  53592.9 &   30.56 &   1.50  &         &        &  53725.8 &  45.84 &   2.34 &        &        &\\
             &  55379.5 &   32.70 &   0.96  &  -1.20  &  0.08  &  55379.5 &  43.63 &   3.55 &   0.52 &   0.05 &\\
 PG 0043+039 &  53381.3 &   14.28 &   1.55  &         &        &  53381.3 &  22.14 &   2.03 &        &        &\\
             &  55383.0 &   16.03 &   0.55  &  -1.06  &  0.13  &  55382.0 &  25.22 &   2.12 &  -1.05 &   0.15 &\\
 PG 0049+171 &  53750.4 &   13.60 &   0.99  &         &        &  53750.4 &  19.02 &   2.40 &        &        &\\
             &  55342.6 &   15.76 &   0.34  &  -2.07  &  0.17  &  55342.6 &  17.96 &   1.17 &   0.40 &   0.06 &\\
 PG 0050+124 &  53011.3 &  478.15 &   9.13  &         &        &  53011.3 & 892.90 &  19.03 &        &        &\\
             &  55387.5 &  455.92 &   5.68  &   2.07  &  0.05  &  55387.5 & 846.07 &  16.40 &   1.86 &   0.06 &\\
 PG 0052+251 &  53008.5 &   41.71 &   3.08  &         &        &  53008.5 &  78.37 &   5.12 &        &        &\\
             &  55355.5 &   43.90 &   0.67  &  -0.69  &  0.06  &  55355.5 &  74.85 &   1.86 &   0.65 &   0.05 &\\
 PG 0157+001 &  53011.0 &  110.41 &   2.76  &         &        &  53011.0 & 417.35 &   7.25 &        &        &\\
             &  55321.3 &  105.61 &   1.52  &   1.53  &  0.05  &  55321.3 & 420.54 &   6.78 &  -0.32 &   0.01 &\\
 PG 0804+761 &  53065.9 &  145.86 &   3.28  &         &        &  53065.9 & 209.84 &   4.96 &        &        &\\
             &  55284.5 &  157.65 &   2.11  &  -3.02  &  0.09  &  55284.5 & 195.44 &   3.77 &   2.31 &   0.08 &\\
 PG 0838+770 &  53348.4 &   29.68 &   1.57  &         &        &  53654.1 &  69.12 &   1.93 &        &        &\\
             &  55286.8 &   30.88 &   0.50  &  -0.73  &  0.04  &  55286.8 &  67.76 &   1.95 &   0.49 &   0.02 &\\
 PG 0844+349 &  53687.9 &   50.57 &   2.37  &         &        &  53716.8 &  90.86 &   3.08 &        &        &\\
             &  55305.5 &   56.45 &   0.88  &  -2.33  &  0.13  &  55305.5 &  94.49 &   2.52 &  -0.91 &   0.04 &\\
 PG 0921+525 &  53875.4 &   63.90 &   2.21  &         &        &  53875.4 &  91.86 &   2.66 &        &        &\\
             &  55306.8 &   75.66 &   1.15  &  -4.73  &  0.20  &  55306.8 &  97.95 &   2.71 &  -1.60 &   0.07 &\\
 PG 0923+201 &  53692.9 &   34.37 &   2.67  &         &        &  53717.0 &  47.81 &   2.36 &        &        &\\
             &  55319.5 &   41.77 &   0.68  &  -2.68  &  0.23  &  55319.5 &  50.65 &   1.96 &  -0.93 &   0.06 &\\
 PG 0923+129 &  53881.0 &  117.79 &   2.86  &         &        &  53881.0 & 225.18 &   4.50 &        &        &\\
             &  55321.7 &  127.44 &   1.71  &  -2.90  &  0.09  &  55321.7 & 228.35 &   5.34 &  -0.45 &   0.02 &\\
 PG 0934+013 &  53880.9 &   36.37 &   1.20  &         &        &  53880.9 &  78.34 &   2.44 &        &        &\\
             &  55327.8 &   32.76 &   0.83  &   2.49  &  0.12  &  55327.8 &  70.44 &   3.50 &   1.85 &   0.12 &\\
 PG 0947+396 &  53716.9 &   28.10 &   1.06  &         &        &  53716.9 &  46.57 &   1.97 &        &        &\\
             &  55318.0 &   31.05 &   0.48  &  -2.54  &  0.11  &  55318.0 &  49.50 &   1.77 &  -1.11 &   0.07 &\\
 PG 0953+414 &  53112.1 &   30.74 &   3.23  &         &        &  53112.1 &  44.57 &   4.72 &        &        &\\
             &  55318.3 &   35.39 &   0.61  &  -1.42  &  0.16  &  55318.3 &  44.48 &   1.72 &   0.02 &   0.00 &\\
 PG 1001+054 &  53512.7 &   23.23 &   2.10  &         &        &  53714.7 &  34.54 &   2.54 &        &        &\\
             &  55332.6 &   27.70 &   0.54  &  -2.06- &  0.21  &  55332.6 &  36.12 &   1.41 &  -0.55 &   0.05 &\\
 PG 1004+130 &  53715.1 &   41.15 &   1.65  &         &        &  53715.1 &  73.63 &   3.53 &        &        &\\
             &  55330.7 &   41.77 &   0.70  &  -0.35  &  0.02  &  55330.7 &  74.99 &   2.48 &  -0.32 &   0.02 &\\
 PG 1011-040 &  53908.9 &   50.33 &   2.01  &         &        &  53908.9 & 100.24 &   3.23 &        &        &\\
             &  55340.6 &   52.49 &   0.80  &  -1.00  &  0.05  &  55340.5 & 100.51 &   2.38 &  -0.07 &   0.00 &\\
 PG 1012+008 &  54088.6 &   31.61 &   1.47  &         &        &  54088.6 &  54.01 &   2.89 &        &        &\\
             &  55338.0 &   32.28 &   0.90  &  -0.39  &  0.02  &  55338.2 &  53.78 &   3.76 &   0.05 &   0.00 &\\
 PG 1022+519 &  53881.7 &   25.45 &   1.05  &         &        &  53881.7 &  42.38 &   2.06 &        &        &\\
             &  55318.3 &   31.17 &   0.56  &  -4.79  &  0.24  &  55318.3 &  44.57 &   1.39 &  -0.88 &   0.06 &\\
 PG 1048+342 &  53881.8 &   14.01 &   0.85  &         &        &  53881.8 &  25.98 &   2.02 &        &        &\\
             &  55332.4 &   15.71 &   0.32  &  -1.86  &  0.13  &  55332.4 &  24.88 &   1.05 &   0.49 &   0.05 &\\
 PG 1048-090 &  53908.9 &   11.56 &   0.89  &         &        &  53908.9 &  20.80 &   1.99 &        &        &\\
             &  55350.8 &   12.21 &   0.31  &  -0.70  &  0.06  &  55350.8 &  21.35 &   1.28 &  -0.23 &   0.03 &\\
 PG 1049-005 &  53723.5 &   45.98 &   1.66  &         &        &  53723.5 &  94.97 &   3.43 &        &        &\\
             &  55347.7 &   47.26 &   0.80  &  -0.69  &  0.03  &  55347.7 &  96.61 &   2.68 &  -0.37 &   0.02 &\\
 PG 1100+772 &  53326.5 &   26.72 &   1.79  &         &        &  53326.5 &  44.60 &   2.48 &        &        &\\
             &  55297.3 &   27.19 &   0.43  &  -0.26  &  0.02  &  55297.3 &  46.37 &   1.41 &  -0.62 &   0.04 &\\
 PG 1103-006 &  53755.6 &   17.65 &   2.26  &         &        &  53755.6 &  31.70 &   2.53 &        &        &\\
             &  55351.0 &   18.54 &   0.39  &  -0.39  &  0.05  &  55351.0 &  32.08 &   1.40 &  -0.13 &   0.01 &\\
 PG 1114+445 &  53881.8 &   68.72 &   2.67  &         &        &  53881.8 & 133.28 &   2.92 &        &        &\\
             &  55332.0 &   70.35 &   1.00  &  -0.57  &  0.03  &  55332.0 & 133.11 &   3.32 &   0.04 &   0.00 &\\
 PG 1115+407 &  53881.8 &   22.99 &   1.41  &         &        &  53881.8 &  40.43 &   1.95 &        &        &\\
             &  55334.3 &   27.91 &   0.47  &  -3.30  &  0.23  &  55334.3 &  44.36 &   1.41 &  -1.63 &   0.11 &\\
 PG 1116+215 &  53139.3 &   80.75 &   6.98  &         &        &  53139.3 & 114.27 &   8.85 &        &        &\\
             &  55345.2 &   81.00 &   1.27  &  -0.04  &  0.00  &  55345.2 & 105.34 &   3.04 &   0.95 &   0.09 &\\
 PG 1119+120 &  53138.2 &  106.13 &   3.19  &         &        &  53138.2 & 218.42 &   7.91 &        &        &\\
             &  55349.6 &  115.16 &   1.62  &  -2.52  &  0.09  &  55349.6 & 220.09 &   4.62 &  -0.18 &   0.01 &\\
 PG 1121+422 &  53723.0 &   10.18 &   0.87  &         &        &  53723.0 &  13.00 &   1.71 &        &        &\\
             &  55334.5 &   11.41 &   0.27  &  -1.34  &  0.13  &  55334.5 &  12.23 &   0.78 &   0.41 &   0.07 &\\
 PG 1126-041 &  53551.8 &  122.73 &  14.731 &         &        &  53749.7 & 246.56 &   4.74 &        &        &\\
             &  55357.4 &  135.92 &   1.97  &  -0.89  &  0.12  &  55357.4 & 247.86 &   5.15 &  -0.19 &   0.01 &\\
 PG 1149-110 &  53551.6 &   48.30 &   2.13  &         &        &  53551.6 & 114.40 &   3.11 &        &        &\\
             &  55364.9 &   47.87 &   0.82  &   0.19  &  0.01  &  55364.9 & 109.50 &   2.65 &   1.20 &   0.05 &\\
 PG 1151+117 &  52990.8 &   20.16 &   5.54  &         &        &  52990.8 &  29.32 &   7.42 &        &        &\\
             &  55356.8 &   17.98 &   0.34  &   0.39  &  0.13  &  55356.8 &  27.68 &   1.34 &   0.22 &   0.06 &\\
 PG 1202+281 &  53908.5 &   34.92 &   1.57  &         &        &  53908.5 &  78.41 &   2.47 &        &        &\\
             &  55352.1 &   33.49 &   0.57  &   0.86  &  0.05  &  55352.1 &  77.95 &   1.91 &   0.15 &   0.01 &\\
 PG 1211+143 &  53011.9 &  151.62 &   3.49  &         &        &  53011.9 & 264.30 &   7.31 &        &        &\\
             &  55360.6 &  149.31 &   2.00  &   0.57  &  0.02  &  55360.6 & 244.46 &   5.70 &   2.14 &   0.09 &\\
 PG 1216+069 &  53753.8 &   16.02 &   1.14  &         &        &  53753.8 &  23.24 &   2.30 &        &        &\\
             &  55364.1 &   18.83 &   0.38  &  -2.34  &  0.19  &  55364.1 &  21.55 &   1.30 &   0.64 &   0.09 &\\
 PG 1226+023 &  54883.7 &  369.60 &   5.95  &         &        &  54883.7 & 650.55 &  11.06 &        &        &\\
             &  55370.4 &  323.66 &   4.09  &   6.37  &  0.15  &  55370.4 & 500.96 &   9.52 &  10.25 &   0.33 &  variable, FSRQ\\
 PG 1229+204 &  53558.5 &   63.65 &   3.06  &         &        &  53766.2 & 141.40 &   3.81 &        &        &\\
             &  55361.9 &   66.20 &   0.95  &  -0.80  &  0.04  &  55361.9 & 142.76 &   3.33 &  -0.27 &   0.01 &\\
 PG 1244+026 &  53766.3 &   44.81 &   1.59  &         &        &  53766.3 &  98.65 &   3.47 &        &        &\\
             &  55374.2 &   47.92 &   0.77  &  -1.76  &  0.08  &  55374.2 & 102.85 &   2.44 &  -0.99 &   0.05 &\\
 PG 1259+593 &  53760.2 &   20.13 &   0.81  &         &        &  53760.2 &  21.25 &   1.52 &        &        &\\
             &  55339.2 &   21.96 &   0.40  &  -2.03  &  0.10  &  55339.2 &  20.73 &   1.00 &   0.29 &   0.03 &\\
 PG 1302-102 &  53417.3 &   42.62 &   1.85  &         &        &  53765.0 &  91.90 &   2.94 &        &        &\\
             &  55304.0 &   43.22 &   0.68  &  -0.31  &  0.02  &  55304.0 &  93.89 &   2.41 &  -0.52 &   0.02 &  FSRQ\\
 PG 1307+085 &  53753.9 &   33.65 &   5.79  &         &        &  53753.9 &  74.14 &   7.91 &        &        &\\
             &  55344.7 &   37.75 &   0.60  &  -0.70  &  0.13  &  55344.7 &  69.02 &   2.27 &   0.62 &   0.08 &\\
 PG 1309+355 &  53139.3 &   52.29 &   5.57  &         &        &  53139.3 & 113.49 &   6.49 &        &        &\\
             &  55362.9 &   49.58 &   0.75  &   0.48  &  0.06  &  55362.9 & 105.34 &   2.53 &   1.17 &   0.08 &  FSRQ\\
 PG 1310-108 &  53764.9 &   71.24 &   1.77  &         &        &  53764.9 & 126.51 &   3.91 &        &        &\\
             &  55297.7 &   74.69 &   1.02  &  -1.69  &  0.05  &  55297.7 & 124.57 &   2.91 &   0.40 &   0.02 &\\
 PG 1322+659 &  53907.0 &   25.12 &   0.91  &         &        &  53907.0 &  43.76 &   1.78 &        &        &\\
             &  55331.1 &   26.33 &   0.45  &  -1.20  &  0.05  &  55331.1 &  43.51 &   1.54 &   0.11 &   0.01 &\\
 PG 1341+258 &  53753.9 &   20.97 &   1.23  &         &        &  53753.9 &  41.70 &   1.89 &        &        &\\
             &  55309.6 &   22.66 &   0.41  &  -1.31  &  0.09  &  55309.6 &  42.17 &   1.28 &  -0.21 &   0.01 &\\
 PG 1351+236 &  53753.9 &   26.47 &   1.09  &         &        &  53753.9 &  48.88 &   2.09 &        &        &\\
             &  55350.2 &   29.27 &   0.52  &  -2.32  &  0.12  &  55350.2 &  50.37 &   1.54 &  -0.57 &   0.03 &\\
 PG 1351+640 &  53112.8 &  161.66 &   3.43  &         &        &  53112.8 & 418.73 &   7.46 &        &        &\\
             &  55340.0 &  173.82 &   2.32  &  -2.94  &  0.08  &  55340.0 & 410.59 &   7.82 &   0.75 &   0.02 &\\
 PG 1352+183 &  53755.7 &$\cdots$ & $\cdots$&         &        &  53755.7 &  31.91 &   6.40 &        &        &\\
             &  55306.7 &   20.80 &   0.37  & $\cdots$&$\cdots$&  55306.7 &  32.05 &   1.17 &  -0.02 &   0.00 &\\
 PG 1354+213 &  53768.2 &   13.20 &   1.39  &         &        &  53768.2 &  27.48 &   2.10 &        &        &\\
             &  55339.2 &   14.27 &   0.31  &  -0.75  &  0.09  &  55339.2 &  29.69 &   1.24 &  -0.91 &   0.09 &\\
 PG 1402+261 &  53163.7 &   66.09 &   3.92  &         &        &  53163.7 & 105.14 &   5.44 &        &        &\\
             &  55372.4 &   69.20 &   1.02  &  -0.77  &  0.05  &  55372.4 & 103.71 &   2.64 &   0.24 &   0.01 &\\
 PG 1404+226 &  53799.6 &   18.97 &   0.93  &         &        &  53799.6 &  28.14 &   1.92 &        &        &\\
             &  55313.0 &   20.40 &   0.36  &  -1.43  &  0.08  &  55313.0 &  28.99 &   1.27 &  -0.37 &   0.03 &\\
 PG 1411+442 &  53381.7 &   90.40 &   3.34  &         &        &  53381.7 & 122.56 &   2.66 &        &        &\\
             &  55372.8 &  101.04 &   1.50  &  -2.90  &  0.13  &  55372.8 & 120.73 &   2.76 &   0.48 &   0.02 &\\
 PG 1415+451 &  53753.1 &   33.35 &   1.24  &         &        &  53753.1 &  59.01 &   1.91 &        &        &\\
             &  55372.7 &   33.83 &   0.54  &  -0.36  &  0.02  &  55372.7 &  58.16 &   1.64 &   0.34 &   0.02 &\\
 PG 1416-129 &  53597.7 &   14.75 &   1.76  &         &        &  53597.7 &  27.26 &   3.18 &        &        &\\
             &  55321.8 &   13.87 &   0.31  &   0.49  &  0.07  &  55321.8 &  26.88 &   1.16 &   0.11 &   0.02 &\\
 PG 1425+267 &  53803.4 &   20.81 &   1.18  &         &        &  53803.4 &  41.38 &   1.77 &        &        &\\
             &  55316.3 &   21.52 &   0.37  &  -0.58  &  0.04  &  55318.9 &  42.68 &   1.18 &  -0.61 &   0.03 &\\
 PG 1426+015 &  53414.5 &  101.96 &   3.78  &         &        &  53808.4 & 178.19 &   4.00 &        &        &\\
             &  55306.8 &  110.89 &   1.52  &  -2.19  &  0.10  &  55306.8 & 184.93 &   3.62 &  -1.25 &   0.04 &\\
 PG 1427+480 &  53753.2 &   15.74 &   1.18  &         &        &  53753.2 &  40.49 &   1.74 &        &        &\\
             &  55373.0 &   16.36 &   0.30  &  -0.51  &  0.04  &  55373.0 &  41.55 &   1.38 &  -0.48 &   0.03 &\\
 PG 1435-067 &  53563.0 &   28.11 &   2.04  &         &        &  53593.3 &  39.75 &   2.55 &        &        &\\
             &  55319.4 &   29.36 &   0.53  &  -0.59  &  0.05  &  55319.4 &  37.76 &   1.21 &   0.71 &   0.06 &\\
 PG 1440+356 &  53384.5 &   78.60 &   4.56  &         &        &  53813.0 & 165.18 &   2.97 &        &        &\\
             &  55310.6 &   95.08 &   1.39  &  -3.46  &  0.23  &  55310.6 & 174.34 &   3.53 &  -1.99 &   0.06 &\\
 PG 1444+407 &  53753.1 &   34.65 &   1.03  &         &        &  53753.1 &  59.73 &   1.84 &        &        &\\
             &  55309.1 &   37.37 &   0.56  &  -2.31  &  0.09  &  55309.1 &  60.62 &   1.94 &  -0.33 &   0.02 &\\
 PG 1448+273 &  53813.0 &   49.96 &   1.40  &         &        &  53813.0 &  95.75 &   2.74 &        &        &\\
             &  55329.8 &   52.54 &   0.79  &  -1.60  &  0.06  &  55329.8 & 105.05 &   2.38 &  -2.56 &   0.11 &\\
 PG 1501+106 &  53066.7 &  204.58 &   5.26  &         &        &  53066.7 & 438.88 &   7.30 &        &        &\\
             &  55319.5 &  187.80 &   2.44  &   2.90  &  0.10  &  55319.5 & 399.40 &   7.47 &   3.78 &   0.11 &\\
 PG 1512+370 &  53769.3 &   15.66 &   0.82  &         &        &  53769.3 &  29.77 &   1.69 &        &        &\\
             &  55344.8 &   15.97 &   0.31  &  -0.35  &  0.02  &  55344.8 &  30.78 &   0.97 &  -0.52 &   0.04 &\\
 PG 1519+226 &  53595.3 &   40.14 &   2.04  &         &        &  53595.3 &  60.33 &   1.84 &        &        &\\
             &  55335.3 &   41.43 &   0.67  &  -0.60  &  0.03  &  55335.3 &  59.57 &   1.52 &   0.32 &   0.01 &\\
 PG 1534+580 &  53726.5 &   89.20 &   1.93  &         &        &  53726.5 & 176.38 &   3.34 &        &        &\\
             &  55360.9 &   87.44 &   1.21  &   0.77  &  0.02  &  55360.9 & 170.22 &   3.27 &   1.32 &   0.04 &\\
 PG 1535+547 &  53376.2 &   56.98 &   4.94  &         &        &  53376.2 &  75.85 &   2.07 &        &        &\\
             &  55359.2 &   61.73 &   0.90  &  -0.95  &  0.09  &  55359.2 &  73.76 &   1.48 &   0.82 &   0.03 &\\
 PG 1543+489 &  53762.2 &   42.29 &   1.19  &         &        &  53762.2 &  93.44 &   2.35 &        &        &\\
             &  55325.0 &   44.97 &   0.69  &  -1.94  &  0.07  &  55325.0 &  97.77 &   2.27 &  -1.32 &   0.05 &\\
 PG 1545+210 &  53410.2 &   19.68 &   2.69  &         &        &  53410.2 &  35.77 &   3.86 &        &        &\\
             &  55316.5 &   20.42 &   0.36  &  -0.27  &  0.04  &  55316.5 &  35.01 &   1.13 &   0.19 &   0.02 &\\
 PG 1552+085 &  53595.4 &   22.52 &   1.10  &         &        &  53595.4 &  28.52 &   1.79 &        &        &\\
             &  55241.0 &   23.08 &   0.49  &  -0.47  &  0.03  &  55241.0 &  28.38 &   1.28 &   0.06 &   0.01 &\\
 PG 1612+261 &  53598.0 &   41.13 &   1.10  &         &        &  53598.0 &  94.93 &   2.10 &        &        &\\
             &  55241.2 &   42.08 &   0.64  &  -0.74  &  0.02  &  55241.2 &  95.37 &   2.24 &  -0.14 &   0.01 &\\
 PG 1613+658 &  53323.9 &   99.02 &   2.86  &         &        &  53695.1 & 186.75 &   2.93 &        &        &\\
             &  55354.9 &  105.51 &   1.47  &  -2.01  &  0.07  &  55354.9 & 186.47 &   3.07 &   0.07 &   0.00 &\\
 PG 1617+175 &  53444.0 &   38.26 &   2.99  &         &        &  53595.3 &  49.88 &   2.08 &        &        &\\
             &  55245.4 &   43.38 &   0.75  &  -1.66  &  0.15  &  55245.4 &  50.10 &   1.57 &  -0.08 &   0.00 &\\
 PG 1626+544 &  53378.0 &   14.88 &   1.20  &         &        &  53599.1 &  17.41 &   1.30 &        &        &\\
             &  55329.5 &   18.97 &   0.32  &  -3.30  &  0.30  &  55330.5 &  18.19 &   0.73 &  -0.52 &   0.05 &\\
 PG 1700+518 &  53111.5 &   99.67 &   6.76  &         &        &  53111.5 & 181.94 &   8.37 &        &        &\\
             &  55242.9 &   98.38 &   1.15  &   0.19  &  0.01  &  55242.9 & 173.38 &   3.09 &   0.96 &   0.05 &\\
 PG 1704+608 &  53346.9 &   40.48 &   2.59  &         &        &  53346.9 &  97.67 &   4.50 &        &        &\\
             &  55330.3 &   43.98 &   0.62  &  -1.31  &  0.09  &  55330.3 &  97.32 &   1.99 &   0.07 &   0.00 &\\
 PG 2112+059 &  53515.0 &   44.28 &   1.14  &         &        &  53515.0 &  68.53 &   2.03 &        &        &\\
             &  55330.9 &   48.01 &   0.76  &  -2.72  &  0.09  &  55330.9 &  71.09 &   2.04 &  -0.89 &   0.04 &\\
 PG 2130+099 &  53162.6 &  177.30 &   3.91  &         &        &  53162.6 & 312.56 &   6.01 &        &        &\\
             &  55336.4 &  181.17 &   2.50  &  -0.83  &  0.02  &  55336.4 & 299.92 &   5.15 &   1.60 &   0.05 &\\
 PG 2209+184 &  53910.7 &   17.92 &   1.23  &         &        &  53910.7 &  22.50 &   1.76 &        &        &\\
             &  55349.4 &   22.50 &   0.47  &  -3.47  &  0.28  &  55349.4 &  21.37 &   1.33 &   0.51 &   0.06 &  FSRQ\\
 PG 2214+139 &  53324.6 &   76.10 &   2.69  &         &        &  53721.3 &  97.80 &   2.87 &        &        &\\
             &  55348.5 &   82.89 &   1.34  &  -2.26  &  0.10  &  55348.5 &  98.58 &   2.51 &  -0.21 &   0.01 &\\
 PG 2233+134 &  52989.7 &   22.58 &   2.84  &         &        &  52989.7 &  52.11 &   5.20 &        &        &\\
             &  55355.0 &   24.19 &   0.47  &  -0.56  &  0.08  &  55355.0 &  51.40 &   1.90 &   0.13 &   0.01 &\\
 PG 2251+113 &  53349.6 &   24.99 &   2.26  &         &        &  53913.4 &  43.62 &   2.34 &        &        &\\
             &  55358.4 &   28.29 &   0.53  &  -1.43  &  0.14  &  55358.4 &  44.48 &   1.79 &  -0.29 &   0.02 &\\
 PG 2304+042 &  53721.2 &   19.24 &   1.04  &         &        &  53721.2 &  30.09 &   2.79 &        &        &\\
             &  55358.5 &   16.48 &   0.36  &   2.51  &  0.18  &  55358.5 &  25.86 &   1.27 &   1.38 &   0.18 &\\
 PG 2308+098 &  53721.2 &   13.99 &   0.94  &         &        &  53721.2 &  21.70 &   2.13 &        &        &\\
             &  55361.6 &   15.52 &   0.39  &  -1.51  &  0.12  &  55361.6 &  22.21 &   1.29 &  -0.21 &   0.03 &

